PILOT: a balloon-borne experiment to measure the polarized FIR emission of dust grains in the interstellar medium

Future cosmology space missions will concentrate on measuring the polarization of the Cosmic Microwave Background, which potentially carries invaluable information about the earliest phases of the evolution of our universe. Such ambitious projects will ultimately be limited by the sensitivity of the instrument and by the accuracy at which polarized foreground emission from our own Galaxy can be subtracted out. We present the PILOT balloon project which will aim at characterizing one of these foreground sources, the polarization of the dust continuum emission in the diffuse interstellar medium. The PILOT experiment will also constitute a test-bed for using multiplexed bolometer arrays for polarization measurements. We present the results of ground tests obtained just before the first flight of the instrument.

==> GROUND_TEST_DESCRIPTION.tex <==
%\section{GROUND TEST DESCRIPTION}
%\label{sec:GROUNDTESTDESCRIPTION}

%JPB: Moved to Test section
% The aim of the \Pilot ground tests was to validate the instrument behavior and to optimize its performances. These tests were realized in a clean room at the CNES facilities in Toulouse, France. They are described in the next subsections. Since the background falling on the detectors is much stronger in the ground configuration than at ceiling altitude, and the detectors are optimised for a moderate background, of the order of 5 pW/pix, we inserted an additional filter in the filter stack, which attenuates a large fraction of the radiation (by a factor of 20). The transmission of the attenuator was set according to the predictions of a photometric model of the instrument taking into account external and internal sources of emission, as well as the transmission of the various optical filters, as measured at the subsystem level.

%\subsection{Optical performance tests}
%\label{sec:OpticalPerformance}

% For these tests, the \Pilot pointed load was aligned with the IRAP sub-millimeter bench (see the experimental setup in Fig.\,\ref{fig:Conf_test}). The optical bench is composed of a high intensity lamp (Mercury plasma lamp) at the focus of
% a $\rm \phi=1\,m$ diameter Cassegrain telescope, delivering a $1 m$ diameter collimated beam, and acting as a point source at infinite distance. The source is modulated by a rotating chopper. The source is mounted on a motorized 2D moving plate and can be moved at the focus of the system, so that it can be displaced over a limited range without moving the telescope.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.95\linewidth]{./Figures/Conf_test.eps}
% \caption{\footnotesize Configuration of the IRAP sub-mm bench for the focal plane geometry characterization, showing, on the left, the IRAP $\rm \phi=1\,m$ collimator, and on the right, the \Pilot pointed load.
% \label{fig:Conf_test}}
% \end{figure}

%\subsubsection{Optical alignement}
%\label{sec:OpticalAlignement}

%JPB: Moved to the Test section
% The requirement on the overall optical quality of the  \Pilot instrument is that the alignment between the primary mirror and the photometer requires accuracy of the order of $\pm 300 \mu m$ for the focus, and a maximum mismatch of $0,06^\circ $ between optical axes of their optical axes. The requirement must be satisfied at all time during the observations at ceiling altitude, while the elevation of the pointed load is changed and the temperature of the structure evolves. This is actually one of the most stringent requirements for the experiment.

% Fulfilling this requirement has implied a series of actions:

% First, a precise characterisation of the mechanical and optical properties of the primary mirror alone and of the photometer alone have been carried. The mirror characterization \cite{Engel2013} was performed with the submillimeter test bench shown in Fig.\,\ref{fig:Conf_test}.
% The photometer optical characteristics were determined using a ZEMAX simulation and $3D$ measurements.

% Second, specific means and an efficient procedure to align the two subsystems, both in the laboratory and at the launch site, are needed. To perform this alignment, the primary mirror is mounted on an hexapod, which allow six degrees of freedom for the adjustment while maintaining the stiffness of the system. An numerical model of this mechanism allows a fast convergence of the optical alignement. The relative position of the two subsystems is checked by measuring, using a laser tracker system, of a series of optical reference balls associated with the mirror and the photometer.

% Third, despite the fact that the whole structure connecting the photomer and M1, and M1 itself are made of the same material (aluminium), which limits differential dilatation, the optical system is off-axis and no perfect compensation is possible. In order to control the optical alignement during the flight, a thermal model of the instrument has been developed. Before the launch, the use of this model knowing the flight conditions, will allow to correct for the expected displacement, compensating to first order the effect of the thermal expansion of the mechanical structure expected at ceiling altitude.

% %This could actually be with point two ...
% Fourth, deformation of the holding structure due to gravity at the various elevations of the pointed load have been modeled (using a finite elements analysis based on Nastram). The deformations are expected to be somewhat lower than thermal deformations. They have also been measured during tests.

%\subsubsection{Defocusing tests}
%\label{sec:DefocusingTests}

% In order to determine the best optical alignement of M1 with respect to the photometer, we have performed a series of defocusing along three orthogonal axes, around the best theorical focus supplied by the Zemax model. The Z defocusing direction corresponds to the optical axis of the photometer while X and Y are orthogonal to it.
% To estimate impact of defocusing on the optical performance, several parts of the focal plane have been explored with the colimator  for each defocus. We performed source micro-scanning where the position of the source is changed by a fraction of the detector pixels, allowing a better determination of the source Point Spread Function (PSF).
% The source PSF  was fitted in the obtained images, in order to measure the changes in the Full Width Half Maximum (FWHM) and encircled energy as a function of defocusing distance. 
% The best focus position was determined as the position of minimum PSF FWHM.

% \subsection{Focal plane geometry}
% \label{sec:FocalPlaneGeometry}

% The aim of this test is to establish the precise correspondance between positions in the focal plane and directions in the sky.
% For this test, the sub-millimeter bench (shown in Fig.\,\ref{fig:Conf_test}) calibrated
% %in order to de the elevation angle and the cross-elevation angle source moving. 
% using a theodolit to provide the correspondance between source deplacement at the focus of the bench $( X,Y )$ and the elevation and cross elevation offsets of the source $(\Delta_{el} ; \Delta_{cel})$ direction. 
% The source has been scanned over a set of position on each array of the instrument. Each $( X,Y )$ position of the source have been located (with their elevation angle and their cross-elevation angle in relation to the center of the instrument focal plane), dated by the on board computer and saved with the data. 
% This exploration provide the instrument focal plane geometry.

%\subsection{polarization}
%\label{sec:polar}

% In order to characterize the polarization performances of the experiment, we use a large format ($\rm 1 \times 1\,m$) polarizer, developed originally for the \Archeops experiment. The polarizer is composed of an array of $3 \times 3$ frames hosting a large number of metal wires ($50\mic$ thickness, $100\mic$ separation). The polarizer is inserted in the beam of the collimator as shown in Fig.\,\ref{fig:conf_test_ARPOB}, and can be rotated, in order to produce a polarized source with any polarization direction. Assuming that polarization cross talk of the PILOT instrument is negligible, the polarizer was shown to provide a source polarization fraction higher than $73\%$ in the \Pilot $240\mic$ band.

% The wire direction of each frame constituting the whole polarizer were measured with theodolits and laser-tracker. The medium wire,  orthogonal to the polarization direction, was measured in relation with the polariser mechanical structure with a précision about $2.4 arcminutes$. A series of optical reference balls associated with the polarizer structure allow its orientation with an accuracy of $1.4 arcseconds$.  The porarization beam direction in relation to the instrument is known with a precision about $2.4 arcminutes$.

%\subsubsection{Instrumental polarization}
%\label{sec:InstrumentalPolarization}

% Optical calculations show that the direction of an incident linear polarization can be slightly rotated through the optics, as it propagates from the primary mirror to the detector. This rotation angle varies accross the focal-plane, and, according to calculations, can reach a few degrees away from the optical axis. This rotation must be measured precisely and taken into account during astronomical data processing. 
% To characterize this rotation, the whole focal plane has been scanned with the polarizer set at different polarization directions, in order to measure the polarization distortion. For each position, the direction of the polarizer has been measured with respect to the instrument, using a laser-tracker system, with an accuracy better than $?"$.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.95\linewidth]{./Figures/conf_test_ARPOB.eps}
% \caption{\footnotesize Optical bench used to characterize polarization properties of the instrument, showing from left to right, the IRAP $\rm \phi=1\,m$ collimator, the large format \Archeops polarizer and the \Pilot pointed load.
% \label{fig:conf_test_ARPOB}}
% \end{figure}

% \subsubsection{Half wave plate characterization}
% \label{sec:HalfWavePlateCharacterization}

% In order to characterize the half wave plate, measurements with the \Archeops polarizer in various positions were done (picture of the configuration shown in fig \,\ref{fig:conf_test_ARPOB}).

% \noindent Two kinds of measurements have been realized :
% \begin{itemize}
% 	\item The HWP is maintained fixed and the Archeops polarizer is rotated. 
% 	\item The Archeops polarizer is maintained fixed and the HWP is rotated.
% \end{itemize}


% \subsection{Background measurement}
% \label{sec:BackgroundMeasurement}

% The aim of these tests is to measure the amplitude and spatial shape of the background. These measurements are also used to derive the electronic offsets of the detectors and to measure the instrumental polarization. For these tests, the experience has been placed under a controled Nitrogen atmosphere (relative humidity $ < 2 \%$) in order to diminish absorption between the emission source and the instrument, which is mostly contributed by water in the atmosphere. 

% \noindent Three configurations were used for these tests:
% First, a $1 m^2$ ecosorb sheet, acting as a room temperature black body, was placed in front of the whole instrument, covering the whole  the whole instrument field of view.
% Second, the \Pilot primary mirror was removed and a tank containing eccosorb maintained either at room temperature or at Liquid Nitrogen ($77 K$) temperature was inserted in from of the photometer, agin covering the whole FOV of the instrument.

% \begin{figure}[htb]
% \centering
% \includegraphics[width=0.95\linewidth]{./Figures/cdp.eps}
% \caption{\footnotesize Cryogenic mirror system, showing, from left to right, the optical design, the spheric mirror and the whole cryogénic mirror system under duriong the tests.
% \label{fig:cdp}}
% \end{figure}

% Finally, a spherical reflecting structure was placed just in front of the entrance window of the photometer, as shown in Fig.\,\ref{fig:cdp}, so that no background from the room enters the system and the instrument sees it self in reflection. This mirror can cooled at $77 K $, in order to reduce further reduce  its contribution to the background. The goal of this last experiment is to prepare a functional test of the detectors on the launch site, once the attenuator has been removed from the instrument, but the background is still much higher than that expcted in flight.






